Non-Equilibrium Statistical Mechanics of Strongly Anharmonic Chains of Oscillators

We study the model of a strongly non-linear chain of particles coupled to two heat baths at different temperatures. Our main result is the existence and uniqueness of a stationary state at all temperatures. This result extends those of Eckmann, Pillet, Rey-Bellet to potentials with essentially arbitrary growth at infinity. This extension is possible by introducing a stronger version of H\"ormander's theorem for Kolmogorov equations to vector fields with polynomially bounded coefficients on unbounded domains.

==> ChainFig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	 LaTeX file generated by Martin's Grapher Library !
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newdimen\MHpointsize
\newdimen\MHpicturesize
\MHpointsize=1pt
\MHpicturesize=374.22pt

\multiply\MHpointsize by \scalep
\divide\MHpointsize by \scaleq
\multiply\MHpicturesize by \scalep
\divide\MHpicturesize by \scaleq

\setlength{\unitlength}{\MHpointsize}
\begin{center}
  \begin{picture}(0,0)
    \epsfig{file=ChainFig.1.ps,width=\MHpicturesize}
  \end{picture}
  \begin{picture}(374.22,124.74)
    \put(70.875,41.391){\llap{$q_0$}}
    \put(104.895,87.885){$V_2(\tilde q_1)$}
    \put(106.312,36.855){$V_1(q_0)$}
    \put(301.928,41.391){$q_N$}
    \put(28.35,87.885){$T_{\!L}$}
    \put(338.783,87.885){\llap{$T_{\!R}$}}
  \end{picture}
\end{center}


==> Func.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	 LaTeX file generated by Martin's Grapher Library !
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newdimen\MHpointsize
\newdimen\MHpicturesize
\MHpointsize=1pt
\MHpicturesize=141.75pt

\newdimen\MHlength
\multiply\MHpointsize by \scalep
\divide\MHpointsize by \scaleq
\multiply\MHpicturesize by \scalep
\divide\MHpicturesize by \scaleq

\setlength{\unitlength}{\MHpointsize}
\begin{center}
  \begin{picture}(0,0)
    \epsfig{file=Func.1.ps,width=\MHpicturesize}
  \end{picture}
\MHlength=2.5pt
  \begin{picture}(141.75,85.05)(\the\MHlength plus 0,0)
      \settowidth{\MHlength}{$\phi(x)$}
      \divide\MHlength by2
    \put(70.875,65.0382){\hspace{-\MHlength}$\phi(x)$}
  \end{picture}
\end{center}


==> SpectrFig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%	 LaTeX file generated by Martin's Grapher Library !
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newdimen\MHpointsize
\newdimen\MHpicturesize
\MHpointsize=1pt
\MHpicturesize=158.76pt

\newdimen\MHlength
\multiply\MHpointsize by \scalep
\divide\MHpointsize by \scaleq
\multiply\MHpicturesize by \scalep
\divide\MHpicturesize by \scaleq

\setlength{\unitlength}{\MHpointsize}
\begin{center}
  \begin{picture}(0,0)
    \epsfig{file=SpectrFig.1.ps,width=\MHpicturesize}
  \end{picture}
\MHlength=2.5pt
  \begin{picture}(158.76,136.08)(\the\MHlength plus 0,0)
      \settowidth{\MHlength}{$\Im \lambda$}
      \divide\MHlength by2
    \put(45.36,124.74){\hspace{-\MHlength}$\Im \lambda$}
    \put(137.214,64.9782){$\Re \lambda$}
  \end{picture}
\end{center}

